Exploring End-to-End Multi-channel ASR with Bias Information for Meeting Transcription

Joint optimization of multi-channel front-end and automatic speech recognition (ASR) has attracted much interest. While promising results have been reported for various tasks, past studies on its meeting transcription application were limited to small scale experiments. It is still unclear whether such a joint framework can be beneficial for a more practical setup where a massive amount of single channel training data can be leveraged for building a strong ASR back-end. In this work, we present our investigation on the joint modeling of a mask-based beamformer and Attention-Encoder-Decoder-based ASR in the setting where we have 75k hours of single-channel data and a relatively small amount of real multi-channel data for model training. We explore effective training procedures, including a comparison of simulated and real multi-channel training data. To guide the recognition towards a target speaker and deal with overlapped speech, we also explore various combinations of bias information, such as direction of arrivals and speaker profiles. We propose an effective location bias integration method called deep concatenation for the beamformer network. In our evaluation on various meeting recordings, we show that the proposed framework achieves a substantial word error rate reduction.

==> tex/sharemask.tex <==
\section{Efficient use of mask estimation}

\begin{figure*}[tb]
\begin{centering}
\includegraphics[scale=0.42]{figure/sharedmask.pdf}
\caption{Mask estimation using various strategies. (a) Conventional structure: separately expert networks for neural WPE and neural MVDR, respectively; (b) MaskNet1: share the whole network (c) MaskNet2: share shallow BLSTM layer; (d) MaskNet3: share BLSTM layers.}
\label{fig:sharenet}
\end{centering}
\vspace*{-4mm}
\end{figure*}

ASR systems are usually trained on representative and dimension-reduced features (e.g. MFCC, PLP, and filter-bank features), avoiding using redundant information from speech signals. 
However, in the ME2E system, representations of all the time-frequency bins are important to reconstruct the noise-free or reverberation-free signals internally, which means a more complex network has been introduced. 
In the front-end processing, using an expert neural network for respective mask estimation is straight-forward but computation consuming. 
Time-frequency masks of WPE and MVDR have their own identities, while essentially, they share common properties - belonging to speech or non-speech.  
In order to make more efficient use of the neural network for mask estimation, shared structures have been investigated in this section instead of using both {\bf DereverbNet} and {\bf BeamformNet} in \cite{subramanian2019dry}.
Three structures have been explored as shown in Fig.\ref{fig:sharenet}.

\subsection{Share the whole network}
Fig.\ref{fig:sharenet} (b) shows a fully sharing structure for WPE and MVDR, which assumes that speech masks and noise masks for dereverberation and beamforming are identical. A typical two-layer BLSTMp (BLSTM with a projection layer) network is given followed by a Linear affine layer and a Sigmoid layer that scaling the outputs between 0 and 1 (denoted by MaskNet1).
Masks estimated from this network are given by:
\begin{equation}
\label{eqn:sharewpe}
M_{v} (t, f, m) = \text{MaskNet1}_{v}(y(t, f, m)) \  v \in \{\text{S}, \text{N}\} 
\end{equation}
Speech mask is for estimating power magnitue spectrum of each channel in WPE-based dereverberation (Eq.(\ref{eqn:de}))
\begin{equation}
\label{eqn:sharewpe}
M_{\text{dereverb}}(t, f, m) = M_{\text{S}}(t, f, m),
\end{equation}
and both speech and noise masks are for estimating PSDs in MVDR (Eq.(\ref{eqn:psd})):
\begin{equation}
\label{eqn:sharemvdr}
M_v(t,f) = M_v(t, f, m) / M, \  v \in \{\text{S}, \text{N}\}
\end{equation}

By using this fully shared BLSTMp network, parameters used for mask estimation have been reduced to half of the previous structure, which is much efficient.
%as it has already been jointly trained with the encoder-decoder ASR backend. 
Another advantage of the sharing scheme is that the dereverberation and beamforming modules take each other into consideration, further optimizing the common properties of speech signals during training. Visualization of sharing scheme versus separately performing mask estimation will be presented in the discussion part later.

\subsection{Share shallow BLSTM layers}
Inspired by the fully shared structure, it is feasible to only share the shallow BLSTMp layers as shown by Fig.\ref{fig:sharenet} (c), which is denoted by MaskNet2. Dereverberation pays more attention to the direct sound of speeches while beamforming cares more about the speech/noise distinction. They share a majority of features in the time-frequency domain but have slight differences as they have different purposes.
Therefore, a more accurate way is to share some shallow layers in the mask estimation neural network.
In MaskNet2, WPE and MVDR share the first BLSTMp layer. At the second layer, the network splits into two separate BLSTMp sub-networks predicting dereverberation masks and beamforming masks, respectively.
In both sub-networks, speech masks and non-speech masks are predicted simultaneously via noise-aware training, along with all the other modules (including backend ASR) jointly. 
MaskNet2 has one more BLSTMp layer than MaskNet1, but it is still more efficient than the original structure.

\subsection{Share BLSTM layers}
Another option to use sub-networks is illustrated by Fig.\ref{fig:sharenet} (d) (denoted by MaskNet3). In this structure, WPE and MVDR share the BLSTMp layers but keep the final Linear transformation and Sigmoid activation different. The number of parameters in MaskNet3 is between MaskNet1 and Masknet2 if we use a uniform number of units in each layer. Compared with MaskNet2, dereverberation mask and beamforming mask have shared more temporal information in common.
%, as it is usually modeled by the BLSTMp layers.

\subsection{Mask sharing for three front-end modules}
As described above, neural network sharing can save GPU memories and have many other benefits. As same as we proposed, the post-filtering module can also share the mask estimation network with dereverberation and beamforming modules. Since the goals of post-filtering and beamforming are same, we do not split an extra sub-network for post-filtering, which means post-filtering and beamforming share the same speech and noise masks.

